Multiscale Modeling of Colloidal Dynamics in Porous Media: Capturing Aggregation and Deposition Effects

We investigate the influence of multiscale aggregation and deposition on the colloidal dynamics in a saturated porous medium. At the pore scale, the aggregation of colloids is modeled by the Smoluchowski equation. Essentially, the colloidal mass is distributed between different size clusters. We treat these clusters as different species involved in a diffusion-advection-reaction mechanism. This modeling procedure allows for different material properties to be varied between the different species, specifically the rates of diffusion, aggregation, deposition as well as the advection velocities. We apply the periodic homogenization procedure to give insight into the effective coefficients of the upscaled model equations. Benefiting from direct access to microstructural information, we capture by means of 2D numerical simulations the effect of aggregation on the deposition rates recovering this way both the blocking and ripening regimes reported in the literature.

==> minilib.tex <==
\usepackage{xstring}
\usepackage{xargs}
\usepackage{etoolbox}
\makeatletter
% ===constructor=======================================================================================
% 1:   command name
% 2:   glyph
% the new command will function similarly to a dict with error checking
\newcommand\constructor[2]{
  \expandafter\newcommandx\csname #1\endcsname[2][1=,2=]{\ifstrequal{##1}{}
    {#2}
    {\@ifundefined{#1@##1}
      {\errmessage{"#1" has no field named "##1"}}
      {\ifstrequal{##2}{}
        {\@nameuse{#1@##1}}
        {\@ifundefined{\@nameuse{#1@##1}@##2}
          {\errmessage{"\@nameuse{#1@##1}" has no field named "##2"}}
          {\@nameuse{\@nameuse{#1@##1}@##2}}}
      }
    }
  }
  \@namedef{#1@self}{#2}
}
% ———setter————————————————————————————————————————————————————————————————————————
\newcommand\set[3]{             % this, field, value
  \@namedef{#1@#2}{#3}
}
% ———getter————————————————————————————————————————————————————————————————————————
\def\ifstrequalx#1{\edef\@t{#1}\expandafter\ifstrequal\expandafter{\@t}}
\newcommand\cget[2]{\@ifundefined{#1@#2}{\errmessage{"#1" has no field named "#2"}}{\@nameuse{#1@#2}}}
% this one can't be used as argument of other command for some reason
\newcommandx\get[5][3=,4=,5=]{\ifstrequal{#3}{}
  {\cget{#1}{#2}}{\ifstrequal{#4}{}
    {\cget{\cget{#1}{#2}}{#3}}{\ifstrequal{#5}{}
      {\cget{\cget{\cget{#1}{#2}}{#3}}{#4}}
      {\cget{\cget{\cget{\cget{#1}{#2}}{#3}}{#4}}{5}}}}}
\newcommand\self[1]{\@nameuse{#1@self}}
% ===defineDomain======================================================================================
% 1:   command name
% 2:   variable glyph
% 3:   glyph
% 4:   "in" or "on", default is in.
% e.g. \defineDomain{G}{x}{\Gamma}[on]
\newcommandx\defineDomain[4][4=in]{
  \constructor{#1}{#3}                                % e.g. \G:=\Gamma
  \set{#1}{dim}{1}                                    % e.g. \G[dim]:=1
  \set{#1}{domain}{#1}                                % e.g. \G[domain]:=G
  \set{#1}{var}{#2}                                   % e.g. \G[var]:=x
  \set{#1}{on}{#4}                                    % e.g. \G[on]:=on
}
% ———operations————————————————————————————————————————————————————————————————————
% \attachIntegral{G}{\int\int_{\G}}                   % e.g. \int[G]:=\int\int_{\G}
\newcommand\renewInt[2]{
  \set{#1}{int}{#2}
}
% redefine \int to accept one optional argument
\let\oldInt\int
\renewcommandx\int[1][1=]{\ifstrequal{#1}{}
  {\oldInt}
  {\intx{#1}}
}
\newcommand\intx[1]{
  \@ifundefined{#1@int}
  {\int\limits_{\self{#1}}}
  {\@nameuse{#1@int}}
}
% ===defineCrossProduct================================================================================
% 1:   command name
% 2:   domain 1
% 3:   domain 2
% e.g. \defineCrossProduct{TG}{Time}{G}
\newcommand\defineCrossProduct[3]{
  \constructor{#1}{\self{#2}\times\self{#3}}          % \TG:=(0,T)\times\Gamma
  \set{#1}{dim}{2}                                    % \TG[dim]:=2
  \set{#1}{var}{(\get{#2}{var},\get{#3}{var})}        % \TG[var]:=(t,x)
  \set{#1}{d1}{#2}                                    % \TG[1][var]:=(0,T)
  \set{#1}{d2}{#3}                                    % \TG[2][var]:=\Gamma
  \@attachInOn{#1}{#2}{#3}                            % \TG[on]:=on
  \set{#1}{domain}{#1}                                % \TG[domain]:=TG
  \set{#1}{int}{\intx{#2}\intx{#3}}                   % \intx{TG}:=\int_0^T\int_\Gamma
}
% ———getBoundary———————————————————————————————————————————————————————————————————
\newcommand\getBoundaryEx[2]{\@ifundefined{#1@#2}
  {\get{#1}{self}}
  {\get{#1}{#2}}
}
\newcommand\getBoundary[2]{\ifstrequalx{\cget{#1}{dim}}{1} % 1 or 2
  {\cget{#1}{#2}}
  {\getBoundaryEx{\cget{#1}{d1}}{#2}\times\getBoundaryEx{\cget{#1}{d2}}{#2}}
}
% ———ifstrequalx———————————————————————————————————————————————————————————————————
% it's ~ \ifstrequal, except it evaluates its first argument
\def\ifstrequalx#1{\edef\@t{#1}\expandafter\ifstrequal\expandafter{\@t}}
\newcommand\@attachInOn[3]{
  % inherit "on" text with || of #2 and #3
  \@namedef{#1@on}{in}
  \ifstrequalx{\@nameuse{#3@on}}{on}{\@namedef{#1@on}{on}}{}
  \ifstrequalx{\@nameuse{#2@on}}{on}{\@namedef{#1@on}{on}}{}
}
% ===defineBoundarySegment=============================================================================
% e.g. \defineBoundarySegment{G}{A}{Grain}{\Gamma}
\newcommand\defineBoundarySegment[4]{ % boundary, segment type, glyph
  \defineDomain{#1}{\get{#2}{var}}{#4}[on]
  \set{#2}{#3}{#4}
  \set{#2}{ref#3}{#1}
}
\newcommandx\getdomain[2][2=]{\ifstrequal{#2}{}
  {\@nameuse{#1@domain}}
  {\@nameuse{\@nameuse{#1@domain}@d#2}}
}
% ===defineUnknown=====================================================================================
% 1: command name
% 2: glyph
% 3: domain of definition
% e.g. \defineUnknown{temp}{\theta}{TA}
\newcommand\defineUnknown[3]{
  \constructor{#1}{#2}
  \set{#1}{parent}{}
  \set{#1}{domain}{#3}
}
% ———operations————————————————————————————————————————————————————————————————————
% e.g. \attachFlux{coll}{\diff}
\newcommand\attachFlux[2]{
  \set{#1}{coeff}{#2}
}
\newcommand\flux[1]{
  \get{#1}{coeff}\nabla \self{#1}
}
% ===inheritUnknown====================================================================================
% 1: parent
% 2: command name
% 3: glyph
% e.g. \inheritUnknown{coll}{coll_i}{u_i}
\newcommand\inheritUnknown[3]{
  \set{#2}{parent}{#1}
  \set{#2}{self}{#3}
  \set{#2}{domain}{\@nameuse{#1@domain}}
  \set{#2}{vector}{\self{#1}}
}
% ———tdomain———————————————————————————————————————————————————————————————————————
\newcommandx\tdomain[2][2=]{\ifstrequal{#2}{}{\indomain{\cget{#1}{domain}}}
  {\ifstrequal{#2}{1}{\indomain{\cget{\cget{#1}{domain}}{d1}}}
    {\ifstrequal{#2}{2}{\indomain{\cget{\cget{#1}{domain}}{d2}}}
      {\text{on }\getBoundary{\cget{#1}{domain}}{#2}}}}}
% ———indomain——————————————————————————————————————————————————————————————————————
\newcommand\indomain[1]{
  \text{\get{#1}{on} }\get{#1}{self}
}
\makeatother
% ===Lebesgue spaces===================================================================================
\newcommand\Li[1]{
  L^\infty(\self{#1})
}
\newcommand\Lp[1]{
  L^p(\self{#1})
}
\newcommand\Lt[1]{
  L^2(\self{#1})
}
\newcommand\forAll[1]{
  \text{for all }\get{#1}{var}\in\get{#1}{self}
}

==> subsup.tex <==
\usepackage{xargs}
\usepackage{etoolbox}
\newcommand\commajoin[2]{{#1,#2}}
\newcommand\plainjoin[2]{{#1#2}}
\makeatletter
% ===newsubsupcommand==================================================================================
% usage:
% \newsubsupcommand
%   {<command name>}
%   {<variable name>}
%   [{<default subscript>}]       -- defualts to empty
%   [{<default superscript>}]     -- defaults to empty
%   [<subscript join function>]   -- defaults to comma
%   [<superscript join function>] -- defaults to comma
%
% When the defined command is used with a subscript or superscript or both,
% they will be joinded by the appropriate join function to the default sub/super-scripts.
%
% Example:
%
% \newsubsupcommand{\yab}{y}[a][b]
%
% $\yab$      := $y_{a}^{b}$
% $\yab_c$    := $y_{a,c}^{b}$
% $\yab^d$    := $y_{a}^{b,d}$
% $\yab_c^d$  := $y_{a,c}^{b,d}$
%
% \newsubsupcommand{\ya}{y}[a]
% \newsubsupcommand{\yb}{y}[][b]

% \newcommandx\sswrap[5]{
%   #1\sub@sup{#2}{#3}{#4}{5}
% }

\newcommand\newifsubcommand[3]{\newcommand#1{\@ifnextchar_{#2}{#3}}}
\newcommandx\newsubsupcommand[6][3=,4=,5=\commajoin,6=\commajoin]{
  \ifstrequal{#4}{}
  {
    \ifstrequal{#3}{}
    {\newcommand#1{#2}}
    % else
    {\newcommand#1{#2\sub@{#3}{#5}}}
  }
  % else
  {
    \ifstrequal{#3}{}
    {\newcommand#1{#2\sup@{#4}{#6}
      }}
    % else
    {\newcommand#1{#2\sub@sup{#3}{#4}{#5}{#6}}}
  }
}
\def\sub@#1#2{
  \def\default@sub{#1}
  \def\sub@merger{#2}
  \@ifnextchar_
  {\merge@sub}
  {_{\default@sub}}
}
\def\sup@#1#2{
  \def\default@sup{#1}
  \def\sup@merger{#2}
  \@ifnextchar_
  {\plain@sup}
  {\@ifnextchar^
    {\merge@sup}
    {^{\default@sup}}
  }
}
\def\plain@sup_#1{_{#1}
  \@ifnextchar^
  {\merge@sup}
  {^{\default@sup}}
}
\def\sub@sup#1#2#3#4{
  \def\default@sub{#1}
  \def\default@sup{#2}
  \def\sub@merger{#3}
  \def\sup@merger{#4}
  \@ifnextchar_
  {\merge@sub@sup}
  {\@ifnextchar^
    {_{\default@sub}\merge@sup}
    {_{\default@sub}^{\default@sup}}
  }
}
\def\merge@sub_#1{_{\sub@merger{\default@sub}{#1}}}
\def\merge@sup^#1{^{\sup@merger{\default@sup}{#1}}}
\def\merge@sub@sup_#1{_{\sub@merger{\default@sub}{#1}}
  \@ifnextchar^
  {\merge@sup}
  {^{\default@sup}}
}

\def\tail@sup#1#2{
  \def\default@sup{#1}
  \def\sup@merger{#2}
  \@ifnextchar^
  {\merge@sup}
  {^{\default@sup}}
}

% \if@sub{<do this if there's a subscript ahead, \@sub is the subscript in this context>}
%        {<do this otherwise>}

\def\if@sub#1#2{
  \@ifnextchar_{
    \def\@statement{#1}
    \@apply@sub}
  {#2}
}
\def\@apply@sub_#1{\def\@sub{#1}\@statement}


\makeatother
\newsubsupcommand{\yab}{y}[a][b]

